DoUnseen: Tuning-Free Class-Adaptive Object Detection of Unseen Objects for Robotic Grasping

How can we segment varying numbers of objects where each specific object represents its own separate class? To make the problem even more realistic, how can we add and delete classes on the fly without retraining or fine-tuning? This is the case of robotic applications where no datasets of the objects exist or application that includes thousands of objects (E.g., in logistics) where it is impossible to train a single model to learn all of the objects. Most current research on object segmentation for robotic grasping focuses on class-level object segmentation (E.g., box, cup, bottle), closed sets (specific objects of a dataset; for example, YCB dataset), or deep learning-based template matching. In this work, we are interested in open sets where the number of classes is unknown, varying, and without pre-knowledge about the objects' types. We consider each specific object as its own separate class. Our goal is to develop an object detector that requires no fine-tuning and can add any object as a class just by capturing a few images of the object. Our main idea is to break the segmentation pipelines into two steps by combining unseen object segmentation networks cascaded by class-adaptive classifiers. We evaluate our class-adaptive object detector on unseen datasets and compare it to a trained Mask R-CNN on those datasets. The results show that the performance varies from practical to unsuitable depending on the environment setup and the objects being handled. The code is available in our DoUnseen library repository.

==> sections/trash.tex <==
We disucss how datasets for 6D pose estimation can be used for the unseen object classification problem. We introduce how deep network for person re-identificaiton could be used for classification. The processed dataset, the pre-trained network are integrated to into our \textbf{DoUnseen} project

Unseen object segmentation
DoSegment
UOIS
UCN
UOIS

Unseen object classification:
classical non-learning approaches (SIFT/SURF/ORB)
Combining segmentation and classification + ICMERR paper proposed the pipeline for unseen object seg + class


how to use already existing dataset for 6D pose estimation
6D Pose estimation datasets:
offer real dataset
YCB
HomeBrew
LM
DoPose
HOPE

Synthetic datasets

What we introduce in this paper:
- how to parse dataset set for unseen object classification
- Training and evaluating a model on unseen objects
- Integrating this classification model to DoUnseen package

The problem is close to:
- re identification
- Few shot/ one shot
- Prototyping?


All these concepts existed since very long time in face recognition, person re identification. They just were not adopted to object segmentation in robotic grasping

\begin{table*}
    \centering
    \resizebox{\textwidth}{!}
    {
        \begin{tabular}{|c| c|c|c|c|c|c| c|c|c|c|c|c| c|c|c|c|c|c| c|c|c|c|c|c|}
            \hline
                                        & \multicolumn{6}{|c|}{HOPE-real-10-augmented (query good light)} & \multicolumn{6}{|c|}{HOPE-real-10-augmented (query all light)} 
                                        & \multicolumn{6}{|c|}{DoPose-10} & \multicolumn{6}{|c|}{DoPose-10-augmented}\\
            \hline
            Train Dataset     & mAP & R1 & R5 & R10 & R20 & Cluster   & mAP & R1 & R5 & R10 & R20 & Cluster  & mAP & R1 & R5 & R10 & R20 & Cluster  & mAP & R1 & R5 & R10 & R20 & Cluster  \\
            \hline
            \hline
            ImageNet    &27.6&37.5&62.5&73.9&84.8&        &21.7&51.6&68.5&81.5&87.0&         &48.7&70.1&86.9&94.0&97.4&         &47.0&87.2&96.0&97.7&98.8&    \\
            \hline
            YCB         &46.4&60.3&82.1&91.3&95.1&        &43.4&72.3&87.5&93.5&95.7&         &59.4&69.9&84.1&91.6&97.8&         &56.1&78.3&86.4&89.7&92.9&    \\
            \hline
            HomeBrew    &35.0&44.0&67.4&77.7&89.1&        &27.5&53.8&76.6&85.3&93.5&         &54.1&61.5&81.7&88.6&93.4&         &51.1&78.9&89.7&93.4&96.9&    \\
            \hline
            LM          &26.6&31.5&52.7&69.0&77.2&        &23.6&41.3&56.5&66.8&75.0&         &44.0&49.1&66.8&76.8&86.7&         &40.3&64.5&77.1&81.9&86.2&    \\
            \hline
            LM-O        &    &    &    &    &    &        &    &    &    &    &    &         &    &    &    &    &    &         &    &    &    &    &    &    \\
            \hline
            T-Less      &    &    &    &    &    &        &    &    &    &    &    &         &    &    &    &    &    &         &    &    &    &    &    &    \\
            \hline
            \textcolor{red}{DoPose}     &    &    &    &    &    &        &    &    &    &    &    &         &    &    &    &    &    &         &    &    &    &    &    &    \\
            \hline
            Mixed (YCB/HomeBrew/LM)     &40.8&53.8&78.3&88.0&96.2&        &37.8&72.8&90.8&94.6&97.3&         &46.9&59.4&73.5&79.5&88.1&         &36.9&60.9&71.1&75.5&80.7&    \\
            \hline
        \end{tabular}
    }
    \caption{Classification evaluation with CUHK03 metrics on HOPE and DoPose datasets.\\
    \textcolor{red}{I used HOPE as the validation dataset for the training. Does it make any sense to keep it here? or just mentioning that is enough?} \\
    \textcolor{red}{remove from the training datasets. I placed it there just to make sense out of the results}
    \label{tab:classification_results}
    }
\end{table*}

% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Training and Testing configuration}
%     \label{fig:my_label}
% \end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.19\textwidth]{figures/hope_samples/hope_val_sample_0_000000.png}
    \includegraphics[width=0.19\textwidth]{figures/hope_samples/hope_val_sample_0_000001.png}
    \includegraphics[width=0.19\textwidth]{figures/hope_samples/hope_val_sample_0_000002.png}
    \includegraphics[width=0.19\textwidth]{figures/hope_samples/hope_val_sample_0_000003.png}
    \includegraphics[width=0.19\textwidth]{figures/hope_samples/hope_val_sample_0_000004.png}
    \caption{HOPE dataset \cite{tyree2022hope} samples with different light conditions. HOPE-good-light include sample with good light as the first one. HOPE-all includes all samples with all light conditions.}
    \label{fig:hope_samples}
\end{figure}

\begin{table}
    \centering
        \begin{tabular}{|c| c|c|c|c| c|c|c|c|}
            \hline
                        & \multicolumn{4}{|c|}{HOPE} & \multicolumn{4}{|c|}{DoPose} \\
            \hline
            Train Dataset & mAP & R1 & R5 & R10 & mAP & R1 & R5 & R10 \\
            \hline
            \hline
            ImageNet    &    &    &    &        &    &    &    &    \\
            \hline
            YCB         &    &    &    &        &    &    &    &    \\
            \hline
            HomeBrew    &    &    &    &        &    &    &    &    \\
            \hline
            LM          &    &    &    &        &    &    &    &    \\
            \hline
            LM-O        &    &    &    &        &    &    &    &    \\
            \hline
            T-Less      &    &    &    &        &    &    &    &    \\
            \hline
            Mixed       &    &    &    &        &    &    &    &    \\
            \hline
        \end{tabular}
    \caption{Classification evaluation with CMC metrics on HOPE and DoPose datasets.\\}
    \label{tab:classification_results}
\end{table}


\begin{table*}[]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
                   & \multicolumn{6}{|c|}{HOPE 10 all light} & \multicolumn{6}{|c|}{DoPose-20 samples} \\
        \hline
                   & \multicolumn{3}{|c|}{BBox} & \multicolumn{3}{|c|}{Seg} & \multicolumn{3}{|c|}{BBox} & \multicolumn{3}{|c|}{Seg} \\
        \hline
                   & mAP & AP50 & AP75 & mAP & AP50 & AP75 &    mAP & AP50 & AP75 & mAP & AP50 & AP75\\
        \hline
        \hline
        Mask R-CNN                               &\multicolumn{6}{|c|}{NA*}    &    84.5&99.2&96.5 & 74.6&97.0&86.3\\
        \hline
        GT mask + class. (ours)                  &       &      &      &     &      &      &     77.6&77.6&77.6&77.6&77.6&77.6\\
        \hline
        Unseen seg. (FAT 5K)[?] + class. (ours)  &     &      &      &     &     &     &54.0&72.8&65.2&47.8&70.4&56.7\\
        \hline
        UCN [?] + class. (ours)                  &       &      &      &     &      &      &     &    &      &     &      &     \\
        \hline
        UOIS [?] + class. (ours)                 &      &      &      &     &      &      &     &    &      &     &      &     \\
        \hline
    \end{tabular}
    \caption{
    Segmentation and classification evaluation with COCO metrics on HOPE and DoPose dataset using osnet
    }

    % DoPose validation set object occurences: [127, 85, 187, 210, 119, 0, 342, 203, 34, 119, 85, 163, 68, 68, 193, 235, 115, 128]

    
    \label{tab:eval_trained_methods}
\end{table*}


\begin{table}
    \resizebox{0.48\textwidth}{!}
    {
    \centering
        \begin{tabular}{|c| c|c|c|c|c| c|c|c|c|c|}
            \hline
                        & \multicolumn{5}{|c|}{HOPE} & \multicolumn{5}{|c|}{DoPose} \\
            \hline
            Train Dataset & mAP & R1 & R5 & R10 & R20 & mAP & R1 & R5 & R10 & R20 \\
            \hline
            \hline
            ImageNet    &    &    &    &    &        &    &    &    &    &    \\
            \hline
            YCB         &    &    &    &    &        &    &    &    &    &    \\
            \hline
            HomeBrew    &    &    &    &    &        &    &    &    &    &    \\
            \hline
            LM          &    &    &    &    &        &    &    &    &    &    \\
            \hline
            LM-O        &    &    &    &    &        &    &    &    &    &    \\
            \hline
            T-Less      &    &    &    &    &        &    &    &    &    &    \\
            \hline
            Mixed       &    &    &    &    &        &    &    &    &    &    \\
            \hline
        \end{tabular}
    }
    \caption{Evaluation of training of the zero-shot classifier trained on different datasets.\\}
    \label{tab:classifier_training}
\end{table}
